IndustriConnect: MCP Adapters and Mock-First Evaluation for AI-Assisted Industrial Operations

AI assistants can decompose multi-step workflows, but they do not natively speak industrial protocols such as Modbus, MQTT/Sparkplug B, or OPC UA, so this paper presents INDUSTRICONNECT, a prototype suite of Model Context Protocol (MCP) adapters that expose industrial operations as schema-discoverable AI tools while preserving protocol-specific connectivity and safety controls; the system uses a common response envelope and a mock-first workflow so adapter behavior can be exercised locally before connecting to plant equipment, and a deterministic benchmark covering normal, fault-injected, stress, and recovery scenarios evaluates the flagship adapters, comprising 870 runs (480 normal, 210 fault-injected, 120 stress, 60 recovery trials) and 2820 tool calls across 7 fault scenarios and 12 stress scenarios, where the normal suite achieved full success, the fault suite confirmed structured error handling with adapter-level uint16 range validation, the stress suite identified concurrency boundaries, and same-session recovery after endpoint restart is demonstrated for all three protocols, with results providing evidence spanning adapter correctness, concurrency behavior, and structured error handling for AI-assisted industrial operations.

==> generated/tables/tab_stats.tex <==
M1 & Modbus & 30 & 1.4 & 1.5 & 0.8 & 2.0 \\
M2 & Modbus & 30 & 1.6 & 0.8 & 1.3 & 1.9 \\
M3 & Modbus & 30 & 2.9 & 1.0 & 2.6 & 3.3 \\
M4 & Modbus & 30 & 1.5 & 0.9 & 1.2 & 1.8 \\
Q1 & MQTT & 30 & 2.0 & 0.9 & 1.6 & 2.3 \\
Q2 & MQTT & 30 & 1.8 & 0.5 & 1.7 & 2.0 \\
Q3 & MQTT & 30 & 1.8 & 0.6 & 1.6 & 2.0 \\
Q4 & MQTT & 30 & 1.7 & 0.3 & 1.6 & 1.9 \\
O1 & OPC UA & 30 & 3.1 & 0.5 & 2.9 & 3.3 \\
O2 & OPC UA & 30 & 7.8 & 0.8 & 7.5 & 8.1 \\
O3 & OPC UA & 30 & 6.6 & 2.9 & 5.6 & 7.7 \\
O4 & OPC UA & 30 & 104.4 & 2.0 & 103.7 & 105.2 \\
X1 & Cross-protocol & 30 & 7.6 & 0.6 & 7.4 & 7.8 \\
X2 & Cross-protocol & 30 & 7.5 & 1.2 & 7.0 & 7.9 \\
X1p & Cross-protocol & 30 & 4.2 & 1.8 & 3.6 & 4.9 \\
X2p & Cross-protocol & 30 & 3.9 & 0.8 & 3.6 & 4.2 \\


==> generated/tables/tab_stress.tex <==
    \begin{tabularx}{\columnwidth}{@{}llYccc@{}}
        \toprule
        ID & Family & Scenario & SR (\%) & Med. (ms) & p95 (ms) \\
        \midrule
        S1 & Modbus & 4 concurrent reads via Modbus adapter. & 100.0 & 9.9 & 15.2 \\
        S10 & Modbus & Mid-operation mock restart during Modbus reads. & 100.0 & 1727.4 & 1731.7 \\
        S11 & MQTT & Mid-operation mock restart during MQTT reads. & 0.0 & 1751.5 & 1851.3 \\
        S12 & OPC UA & Mid-operation mock restart during OPC UA reads. & 100.0 & 5361.6 & 5373.7 \\
        S2 & MQTT & 4 concurrent reads via MQTT adapter. & 100.0 & 8.9 & 9.8 \\
        S3 & OPC UA & 4 concurrent reads via OPC UA adapter. & 100.0 & 12.2 & 13.4 \\
        S4 & Modbus & Concurrent read + write via Modbus. & 100.0 & 3.2 & 3.6 \\
        S5 & MQTT & Concurrent read + publish via MQTT. & 100.0 & 3.7 & 4.0 \\
        S6 & OPC UA & Concurrent read + write via OPC UA. & 100.0 & 6.4 & 6.7 \\
        S7 & Modbus & 50 sequential rapid-fire reads via Modbus. & 100.0 & 64.5 & 86.0 \\
        S8 & MQTT & 50 sequential rapid-fire reads via MQTT. & 100.0 & 69.4 & 78.7 \\
        S9 & OPC UA & 50 sequential rapid-fire reads via OPC UA. & 100.0 & 115.9 & 120.5 \\
        \bottomrule
    \end{tabularx}

